Group Membership Verification with Privacy: Sparse or Dense?

Group membership verification checks if a biometric trait corresponds to one member of a group without revealing the identity of that member. Recent contributions provide privacy for group membership protocols through the joint use of two mechanisms: quantizing templates into discrete embeddings and aggregating several templates into one group representation. However, this scheme has one drawback: the data structure representing the group has a limited size and cannot recognize noisy queries when many templates are aggregated. Moreover, the sparsity of the embeddings seemingly plays a crucial role on the performance verification. This paper proposes a mathematical model for group membership verification allowing to reveal the impact of sparsity on both security, compactness, and verification performances. This model bridges the gap towards a Bloom filter robust to noisy queries. It shows that a dense solution is more competitive unless the queries are almost noiseless.

==> introduction.tex <==
% !TEX root = wifs2019_template.tex
\section{Introduction}
Group membership verification is a procedure checking that an item / individual is a member of a group.
The typical scenario is to grant access to a building only to employees working in the facilities.
This task distinguishes members from non-members of the group, but it should not distinguish a member from one another.

During the enrolment, members' templates (biometric traits of individuals or PUF of items) are extracted and aggregated into one compact group representation. The promise here is that the templates are self-protecting each others thanks to the aggregation. There is no need of securing this data structure (homomorphic encryption, fuzzy commitment).  
At verification time, a fresh template is queried. The system decides whether this query is a noisy version of one the enrolled templates or of an unknown template. The access is then granted or refused.

This procedure is similar to the well-known Bloom Filter,
except that BF can not cope with queries which are not an exact copy of the enrolled items.
For this reason, some schemes were proposed in the past~\cite{Gheisari2019icassp, Gheisari_2019_CVPR_Workshops}, based on two mechanisms:
i) the embedding transforms the template into binary or ternary sequences, 
ii) the aggregation blends vectors into one single vector.
These approaches investigate in which order these two mechanisms shall be processed.
The aggregation is based on adhoc signal processing~\cite{Gheisari2019icassp} or learned without supervision~\cite{Gheisari_2019_CVPR_Workshops}.
The embedding is based on the STC scheme~\cite{Razeghi2017wifs,Razeghi2018icassp}.
These papers prove that sparsity is the main ingredient of STC for providing a compact, secure, and privacy enhancing embedding.

This paper studies two questions.
First, the works~\cite{} consider a 1-to-1 identification application, not group membership verification.
Does sparsity help as well in this new application?
Second, the works~\cite{Gheisari2019icassp, Gheisari_2019_CVPR_Workshops} have a severe limitation.
Due to technical constraints, these constructions create highly compact representations, which do not perform well when the size of the group is large. This paper breaks this lock by proposing a scheme allowing to trade compactness for better security or better verification performances.

Sect.~\ref{sec:Setup}  first considers the aggregation of discrete random sequences, and models this compromise with information theoretical tools. Sect.~\ref{sec:Binary} applies this viewpoint to binary random sequences and shows that the noise on the query has an impact depending on the sparsity of the sequences. Sect.~\ref{sec:Real} bridges the gap between the templates, \ie\ real $d$-dimensional vectors, and the discrete sequences considered in the previous sections. Sect.~\ref{sec:Experiments} gathers the experimental results for a group membership verification based on faces.   
 
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "wifs2019_template"
%%% End:

